CineTransfer: Controlling a Robot to Imitate Cinematographic Style from a Single Example

This work presents CineTransfer, an algorithmic framework that drives a robot to record a video sequence that mimics the cinematographic style of an input video. We propose features that abstract the aesthetic style of the input video, so the robot can transfer this style to a scene with visual details that are significantly different from the input video. The framework builds upon CineMPC, a tool that allows users to control cinematographic features, like subjects' position on the image and the depth of field, by manipulating the intrinsics and extrinsics of a cinematographic camera. However, CineMPC requires a human expert to specify the desired style of the shot (composition, camera motion, zoom, focus, etc). CineTransfer bridges this gap, aiming a fully autonomous cinematographic platform. The user chooses a single input video as a style guide. CineTransfer extracts and optimizes two important style features, the composition of the subject in the image and the scene depth of field, and provides instructions for CineMPC to control the robot to record an output sequence that matches these features as closely as possible. In contrast with other style transfer methods, our approach is a lightweight and portable framework which does not require deep network training or extensive datasets. Experiments with real and simulated videos demonstrate the system's ability to analyze and transfer style between recordings, and are available in the supplementary video.

==> 93_Problem_formulation.tex <==
%\subsection{Model Predictive Control problem}
The overall objective of CineTransfer is to record a cinematographic sequence that reproduces the style of another sequence that is given as input of the system, as described in Fig. \ref{fig:main}. The first part of this solution extracts and optimizes the style features from the input sequence and converts them to recording instructions. The instructions are given to the second part which sends commands to a robotic camera that records a scene in a way the output sequence reproduces the style of the input sequence. 
%The second part is built upon CineMPC, 


%. The part that is missing is the first part, extracting the style features of the input sequence is 

%The problem solved in this paper lies in the first part,

A sequence is a succession of frames that represent fixed shots or images. Let $I$ and $O$ represent the input and output sequence, and one frame of them is represented as $I_f$ and $O_f$, respectively, 
\begin{equation}
I = [I_1, I_2, .., I_f, .., I_{nf}], 
\quad
O=[..,O_1, O_2, .., O_f, .., O_{nf},..],
\end{equation}
where $nf$ represents the number of frames from the input sequences whose style is transferred to the output sequence. 
Additionally, let's assume that every sequence has a number of $nt$ main targets that are shown in every frame.

%assuming both sequences have the same number of frames. 


%The overall objective of CineTransfer is to find control commands for a camera and drone to record a scene producing an output sequence, $O$, which reproduces the features of a given input sequence, $I$, as close as possible.


%reproduce the features of an input sequence, , recording scenes producing an output sequence


%obtaining control commands for a camera and drone to record scenes producing an output sequence, $s_o$, that reproduces the features of an input sequence, $s_i$,  as close as possible. 

%The high-level goal is to find the control actions $\mathbf{u}$ for the drone and camera that minimize the difference between the input shot and the output shot for all frames, constrained by the set of constraints $\mathcal{U}_d$,

The high-level goal of this paper is to find the control actions for the drone and camera that minimize the difference between the input and output sequences for all frames. The control actions are the intrinsics and extrinsics of the robotic camera and are grouped into the vector $\mathbf{u}$. These parameters are constrained by the set of constraints $\mathcal{U}$, which depends on the hardware limits of the  cinematographic platform used to record. The optimization problem solved by CineTransfer is described as 
\begin{equation}
\begin{aligned}
\min_{\substack{\mathbf{u}_{1}..\mathbf{u}_{nf}}} \quad & \sum_{f=1}^{nf}{J(O_f,I_f)}\\
\textrm{s.t.} \quad & \mathbf{u}_{f} \in \mathcal{U}\\
  & 
\end{aligned},
\end{equation}
where $J(\cdot,\cdot)$ is a function that extracts cinematographic features of two sequences and penalizes the difference between them. 
The cinematographic features and the details of this function are described in the next sections.
%where $J_{C,f}$ is the cost function of CineTransfer for a particular frame. This cost term 
%Theoretically, there is a function $\varepsilon(\cdot)$, that analyzes the sequences and compares some features from them.
%Therefore, the frame-wise cost function of CineTransfer is expressed as follows,
%\begin{equation}
%J_{C,f} = {\varepsilon(O_f,I_f}),
%    \label{eq:im-cost}
%\end{equation}
%that is expressed between the same frame of the output ($O_f$) and input ($I_f$) sequences.

 


% The input of CineMPC is a set of numerical features that tells the controller how the sequence must be recorded according to the aforementioned factors. However, it can be difficult to determine these values and to give instructions to the platform as some of them are not intuitive to an average user (e.g. exact pixel where to place a target or where to start the depth of field). CineCopy intuitively fills that gap by extracting automatically these features from an input video sequence and converting them to the input format of CineMPC.


% %which receives a set of artistic and technical references as input to autonomously record targets that are present in a scene with a desired depth of field, position of targets in the image and relative recording pose between the targets and the drone.

%SOLUTION

%To achieve this, we need to describe how the features of a sequence are found. Let denote $I$ an input video sequence. CineTransfer extracts the most representative characteristics from $s_i$ and sends commands to control a cinematographic drone to record an output sequence, $s_o$, which is somehow similar to the input sequence $s_i$. 


%The cost function of CineTransfer, can be determined by how close these two features are between the input and output sequences, or the cost associated with the depth of field ($J_{Dof}$) and the cost associated with the framing of the targets in the image, ($J_{\ro}$) for each frame,

% \begin{equation}
% J_{CineTransfer} = \sum_{f=0}^{nf}(J_{Dof,f} + J_{\rho,f}),
% \end{equation}
% which are described in detail in the next subsections.




% This cost term depends on both the intrinsic parameters such as the focal length and the extrinsic parameters -relative pose drone-target-. The term $J_{im}$ is an addition of each element that is present on the scene whose position in the screen is controlled, $\textbf{im}^*=(x,y)$.
% Particularly, in this solution, CineCopy extracts the body joint (e.g. left arm, nose, right ear, etc.) $j$ of each target $t$ that is present on the input video. Thus, $J_{im}$ sums the desired value of each body joint position in pixels of each target, 

% \begin{equation}
% J_{im,k} = \sum_{t=1}^{nt}\sum_{j=1}^{nj}{w_{im,t,j}\left(\textbf{im}_{t,k,j} - \textbf{im}_{t,k,j}^{*}\right)^2}.
%     \label{eq:im-cost}
% \end{equation}
% for all $nt$ targets and its visible body joints $nj$.
 

% discretized the elements in three



% The cost term $J_{DoF}$ is composed of the desired near distance ($Dn^*$) and the far distance ($Df^*$), which are the distances that delimite the depth of field, and its associated weights, $w_{D_{n}}$ and $w_{D_{f}}$, \begin{equation}
% J_{DoF,k} = w_{D_{n}}\left(D_{n,k} - D_{n,k}^{*}\right)^2 + w_{D_{f}}\left(D_{f,k} - D_{f,k}^{*}\right)^2.
%     \label{eq:dof-cost}
% \end{equation}
%  $D_n$ and $D_f$ depend on the intrinsic parameters of the camera; the focal length, the aperture of the lens, and the focus distance.
 
%  In this solution we adjust these distances in terms of the three parts of the scene in which we control the focus; the foreground, the targets, and the background.
%  The near distance ($Dn^*$) is adjusted to the closest target to the drone that should appear in focus. Analogously, the far distance ($Df^*$) is set to the furthest target that should be shown in focus.
%  If the foreground should be in focus, the desired near distance ($Dn^*$) is adjusted to be close to the drone. If the background should appear in focus, the weight associated with the far distance ($Df^*$) is set to 0, so it is not controlled, focusing everything in the scene from the near distance to the background. Moreover, if none of the targets should be in focus, the near and far distances are adjusted to leave the targets out of the depth of field, depending on the desired focus of foreground and background, 
%  \begin{equation}
%   Dn^* =\left\{
%   \begin{array}{@{}ll@{}}
%     0, & \text{if}\ fg.foc=1 \\
%     \min_{\forall foc(t) \in S_t} d(t) & \text{if} \ \exists t \in S_t \rightarrow  t.foc = 1 \\
%     \max_{\forall t \in S_t} d(t) & \text{if} \ \nexists t \in S_t \rightarrow  t.foc = 1 \\ & \wedge\ bg.foc = 1\\
%   \end{array}\right.,
% \end{equation} 
%  \begin{equation}
%   Df^* =\left\{
%   \begin{array}{@{}ll@{}}
%     \infty, & \text{if}\ bg.foc=1 \\
%     \max_{\forall t \in S_t} d(t) & \text{if} \ \exists t \in S_t \rightarrow  t.foc = 1 \\
%     \min_{\forall t \in S_t} d(t) & \text{if} \ \nexists t \in S_t \rightarrow  t.foc = 1 \\ & \wedge\ fg.foc = 1\\
%   \end{array}\right..
% \end{equation} 

% These are determined by the cinematographic platform that we use to control the cinematographic drone to record the scene.  For this purpose, we use and adapt CineMPC \cite{pueyo2022cinempc}.

% CineMPC is an algorithm that solves a non-linear optimization problem inside an MPC (Model Predictive Control) framework to autonomously control a video camera that is embedded in a drone for cinematographic purposes. CineMPC controls three factors of the image; The Depth of Field (DoF), or focus of the image, the position of the elements on the image, and the relative pose between the camera and the targets. 





% In this solution, we extract the features from the input sequence and control the two first factors used by CineMPC, the Depth of Field and the position of the targets on the screen.
% We ignore the relative position between the camera and the target because we assume that all the targets are persons and we know the position of their body joints. Placing the joints in the image will cause the relative rotation between the camera and the target automatically adjusts. Moreover, we avoid controlling the relative distance by controlling the focal length to place the joints in the image, which adjusts the framing of the person on the screen. 

% If the third cost term is discarded, CineMPC optimizes the next cost function at a time step,
% \begin{equation}
% \begin{aligned}
% \min_{\substack{\mathbf{u}_{d,k_0}..\mathbf{u}_{d,k_0+N}\\ \mathbf{u}_{c,k_0}..\mathbf{u}_{c,k_0+N}}} \quad & \sum_{k=k_0}^{k_{0}+N}{J_{DoF,k}
%     + J_{im,k}}\\
% \textrm{s.t.} \quad & \mathcal{C}_k\\
% \end{aligned}, 
% \end{equation}
% to extract the next $N$ drone and camera actions ($\mathbf{u}_{d,k_0+N}$ and $\mathbf{u}_{d,k_0+N}$, respectively) at a giving time $k_0$, and being $\mathcal{C}_k$ the set of constraints about the state and actions of the drone and camera.
%  $J_{DoF}$ and $J_{im}$ are the cost terms associated with the depth of field and the position of the targets in the image. In this solution, these cost terms are adapted as the next subsections explain.
 
% \subsection{Focus of the image - Depth of Field }  %($J_{DoF}$)}
% The depth of field is the part of the scene that appears in focus on screen. The cost term $J_{DoF}$ is composed of the desired near distance ($Dn^*$) and the far distance ($Df^*$), which are the distances that delimite the depth of field, and its associated weights, $w_{D_{n}}$ and $w_{D_{f}}$, \begin{equation}
% J_{DoF,k} = w_{D_{n}}\left(D_{n,k} - D_{n,k}^{*}\right)^2 + w_{D_{f}}\left(D_{f,k} - D_{f,k}^{*}\right)^2.
%     \label{eq:dof-cost}
% \end{equation}
%  $D_n$ and $D_f$ depend on the intrinsic parameters of the camera; the focal length, the aperture of the lens, and the focus distance.
 
%  In this solution we adjust these distances in terms of the three parts of the scene in which we control the focus; the foreground, the targets, and the background.
%  The near distance ($Dn^*$) is adjusted to the closest target to the drone that should appear in focus. Analogously, the far distance ($Df^*$) is set to the furthest target that should be shown in focus.
%  If the foreground should be in focus, the desired near distance ($Dn^*$) is adjusted to be close to the drone. If the background should appear in focus, the weight associated with the far distance ($Df^*$) is set to 0, so it is not controlled, focusing everything in the scene from the near distance to the background. Moreover, if none of the targets should be in focus, the near and far distances are adjusted to leave the targets out of the depth of field, depending on the desired focus of foreground and background, 
%  \begin{equation}
%   Dn^* =\left\{
%   \begin{array}{@{}ll@{}}
%     0, & \text{if}\ fg.foc=1 \\
%     \min_{\forall foc(t) \in S_t} d(t) & \text{if} \ \exists t \in S_t \rightarrow  t.foc = 1 \\
%     \max_{\forall t \in S_t} d(t) & \text{if} \ \nexists t \in S_t \rightarrow  t.foc = 1 \\ & \wedge\ bg.foc = 1\\
%   \end{array}\right.,
% \end{equation} 
%  \begin{equation}
%   Df^* =\left\{
%   \begin{array}{@{}ll@{}}
%     \infty, & \text{if}\ bg.foc=1 \\
%     \max_{\forall t \in S_t} d(t) & \text{if} \ \exists t \in S_t \rightarrow  t.foc = 1 \\
%     \min_{\forall t \in S_t} d(t) & \text{if} \ \nexists t \in S_t \rightarrow  t.foc = 1 \\ & \wedge\ fg.foc = 1\\
%   \end{array}\right..
% \end{equation} 


==> 94B_Features.tex <==

According to literature about cinematography, (~\cite{brown2016cinematography, thompson2009grammar}), two of the main factors that define the style of a shot is the framing of the targets in the scene and the parts of the scene that are shown in focus or out of focus, also called the depth of field.
Therefore, the function that determines the comparison between the features of two frames can be defined as:
\begin{equation}
J(O_f, I_f) = \delta(O_f, I_f) + \eta(O_f, I_f),
\end{equation}
The next subsections define the depth of field and the framing of the targets, as well as the formal definition of a frame for this work.


\subsection{Frame definition}
\label{sec:frame_definition}
 First of all, we need to describe the elements that are present in a frame in order to make comparisons between frames. These elements are the foreground, the background, and the main targets:
\begin{itemize}
  \item Foreground: space between the recording camera to the closest target. We denote the foreground of a frame as $\Gamma_f \in \{\Gamma_0, ..., \Gamma_{nf}\}$.
  \item Main Targets: space of the scene where we find the main $nt$ human targets. Each target of a frame is denoted as $t_{f,t} \in \{t_{0,0}, ..., t_{nf,nt}\}$ and we suppose that the same number of targets are shown along the sequence.
  \item Background: part of the scene between the distance from the farthest target to the infinite. The background of a frame is denoted as $\Delta_f \in \{\Delta_0, ..., \Delta_{nf}\}$
\end{itemize}
Figure \ref{fig:frame} shows a graphical representation of the division of a frame. Fig.\ref{fig:frame}-a shows the raw frame and Fig.\ref{fig:frame}-b shows the frame divided in the foreground (blue), main targets (yellow), and background (red).
\begin{figure}[!h]
\centering
\begin{tabular}{cc}
    \includegraphics[width=0.46\columnwidth]{images/frame21.jpg} 
    &
     \includegraphics[width=0.46\columnwidth]{images/frame21_masked.jpg}
\end{tabular}
\caption{\textbf {Frame division}. (a) Raw image that represents a single frame (b) Frame divided in background (shaded orange part), main targets (shaded yellow part) and  foreground (shaded blue part)}
\label{fig:frame}
\end{figure}


%that are all grouped in the vector $\mathbf{T} = [t_0...t_{nt}]$.
In each frame, each target $t_{f,t}$ is described and characterized with a set of parameters that represent their image localization, their points of interest or body joints, and if it is shown blurred or focused in the image:
\begin{itemize}
  \item $B_{f,t}$: boolean that is true if the target appears in focus and false if it appears blurry. The foreground and background have this attribute too,
  \item  $\mathbf{R}_{f,t} \in \mathbb{R}^{4}$: bounding box of four points (left, right, top, bottom) that represents the region of pixels where the target is placed within the frame, 
  \item  $\mathbf{M}_{f,t}$: mask of booleans that represents the set of pixels where the target is placed on the image, this attribute is also present in the foreground and background,
  \item $\mathbf{P}_{f,t}$: list of $np$ points of interest, $\mathbf{p} = [p_0...p_{np}]$, e.g. head and/or hips of a person. Additionally, each point of interest is categorized by its position on the image $\mathbf{im}_p \in \mathbb{R}^{2}.$
\end{itemize}


\subsection{Focus of the image - Depth of Field - $\delta(\cdot)$}  %($J_{DoF}$)}
The depth of field represents the parts of the scene are in focus or not. It is one aspect of recent' cinematography and depends uniquely on the intrinsincs of the camera (focal length, focus distance and aperture).

The depth of field of a frame is simplified in this solution by only determining if the set of  main targets, the foreground, and the background are in focus or not.

Let $d(\cdot)$ be a function that determines if each element of a frame is in focus or not (e.g. foreground $F_f$ in focus, target $t_{f,1}$ out of focus.) %which is represented by the element's attribute $b$. 
The function $\delta(\cdot)$ compares if all the elements of two frames have the same focus,% using the function $DoF(\cdot)$,

\begin{equation}
\delta(\mathbf{O}_f, \mathbf{I}_f) =  d(\mathbf{O}_f) - d( \mathbf{I}_f).
\end{equation}
Therefore, one of the objectives of CineTransfer is to determine if the elements that compose a %the set of main targets, the background, and the foreground of the 
frame appear focused or blurry in the input sequence.


\subsection{Position of targets in the image - $\eta(\cdot)$}
The framing of a target corresponds to the position of the image where the target appears in a frame.
Thanks to the framing, the image could show a target following some cinematographic rules, e.g. rule of thirds, Cowboy shot.

%The part of the image where the target appears is called the framing of a target.  %The objective of this function is to place the targets in particular regions of the image. 
%As in the previous subsection, there are $nt$ main targets present in a frame, which are represented by the vector $\mathbf{T} = [t_0...t_{nt}]$. Additionally, each target is defined by $np$ points of interest, $\mathbf{p} = [p_0...p_{np}]$, e.g. head and/or hips of a person. 
% The objective of CineTransfer is to place these points of interest in a determinate position of the image of the output sequence in every frame, matching the input video (e.g. in frame 4 there are 2 targets, place the hips of the first target $t_{4,1}$ in the bottom horizontal third of the image, place the left arm of the second target $t_{4,2}$ in the vertical center of the image.).

The objective of CineTransfer is to determine the points of interest in a determinate position of the image of the output sequence in every frame, matching the input video (e.g. in frame 4 there are 2 targets, place the hips of the first target $t_{4,1}$ in the bottom horizontal third of the image, place the left arm of the second target $t_{4,2}$ in the vertical center of the image.).

Let $h(\cdot)$ denote the function that determines the image position in pixels  of all the points of interest of every target of a frame. The function $\eta$ compares the position in the image of all the points of interest of a frame of the input sequence with the position of the same points in the same frame of the output sequence,

\begin{equation}
\eta(\mathbf{O}_f, \mathbf{I}_f) =  h(\mathbf{O}_f) - h( \mathbf{I}_f).
\end{equation}

% \begin{equation}
%  \rho(O_f, I_f) = \sum_{t=0}^{nt} \sum_{p=0}^{np} h(\mathbf{O}_{f,t,p}) - h(\mathbf{I}_{f,t,p}),
% \end{equation}

%where $\mathbf{T'}$ and  $\mathbf{T''}$ represent the set of targets of the frame $f$ in the input sequence and output sequences, respectively.
The framework proposed in CineTransfer should be able to extract all the points of interest of all the main targets that are present in a frame.













==> 95B_Experiments.tex <==
%In this section, we demonstrate CineTransfer's capacity to analyze two input sequences, one from a simulation where we know the ground truth values, and another one from a real movie. Then, we validate the solution using an existing cinematographic drone controller to recreate the real scene in photorealistic simulation.

This section validates CineTransfer's capabilities to \textit{transfer} the style of different input sequences to new automatically acquired recordings in a photo-realistic virtual environment.

The input sequences chosen cover the main aspects to be validated: XXXX (sequence ?), XXXX (sequence ?) and XXXX (sequence ?). This last input sequence is generated in a virtual environment to facilitate quantitative evaluation of ??.

\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c}
                      & Input seq. & Output seq. &  Focus & Main target & Body joints & Target framing \\
         E1 & Sim. & Sim. & TICK & CROSS & \\
         E2 & Real & Sim. \\
         %Experiment 3 & Real & Photorealistic \\
         %Experiment 4 & Real & Photorealistic \\
         
    \end{tabular}
    \caption{Experimental validation}
    \label{tab:my_label}
\end{table}


%The very end of CineTransfer is to control a cinematographic platform by using an input sequence as recording instructions, easing its introduction to users that are not experts. 
%To demonstrate its potential, we present a full experiment whose objective is to reproduce a 

For the simulated sequence, we have recorded a fireman walking in the mountains. In this sequence, the focus of the target changes, and the target is walking, which causes the measures of the body's keypoints be noisy. The sequence is divided into 99 frames that are captured every 0.5 s.
For the real sequence, we have chosen a sequence of 25 s. from the movie "Road to Perdition", awarded the Oscars for best photography in 2003. This sequence is particularly challenging because multiple persons and objects appear, but only one of them is the main target, and there are changes in the depth of field. The sequence is divided into 48 frames that are captured every 0.5 s.

We perform different qualitative and quantitative experiments to demonstrate the capacity of the solution, and we refer the reader to the supplementary video for more complete visual results.


%First, we show how the two sequences are analyzed and the features of the sequence, appropriately optimized. Then, we transform the features into constraints of CineMPC as defined in Sec. \ref{sec_problem_formulation} to recreate the sequence in two different scenarios, and analyze the results.

 \subsection{Implementation details}
 All the experiments are run in Ubuntu 20 on an AMD Ryzen 9 5900X 12-Core CPU equipped with 32 Gb of RAM and an NVidia GeForce GTX 3090 Ti. The pipeline of CineTransfer is implemented in Python. It makes calls to the libraries to detect the focus, the mask, and the position of the targets of the image and collects and optimizes the results, using the Python optimization library Gekko \cite{gekko}, and generate the JSON files. Then, have modified CineMPC which is implemented in ROS and C++ to read the recording instructions from the JSON files.
 
 
 \begin{figure}[!h]
\centering
\begin{tabular}{cc}
    \includegraphics[width=0.48\columnwidth,height=2.1cm]{images/experiment2/pose_1.jpg} 
    &
    
     \includegraphics[width=0.48\columnwidth]{images/experiment2/keypoint.jpg}
    \\ 
    
    \footnotesize (a)  & \footnotesize (d) \\
    
    \includegraphics[width=0.48\columnwidth,height=2.1cm]{images/experiment2/pose_2.jpg} 
    &
    \includegraphics[width=0.48\columnwidth]{images/experiment2/noisy.jpg}
    \\
     \footnotesize (b)  & \footnotesize (e) \\
     
    \includegraphics[width=0.48\columnwidth,height=2.1cm]{images/experiment2/frame0.jpg} 
    &
     \includegraphics[width=0.48\columnwidth]{images/experiment2/focus.jpg}
    \\
     \footnotesize (c)  & \footnotesize (f) \\
\end{tabular}
\caption{\textbf {Analysis of the features of a frame from a simulated sequence.}(a-b) Two subsequent frames of the sequence showing the skeleton for the body joints detection algorithm (c) Focus map detected by the focus detection measure. White areas are focused, and black areas are out of focus. (d) Plot showing the ground truth (light color) and CineTransfer values for the point of the chest of the target (red middle point in skeleton). Blue are vertical components and Orange are horizontal components (e) Vertical component of the chest of the target when the continuity between frames is not optimized (light) and when it is (dark) (f) Evolution of the detected focus of the main target. Light color is the percentage of pixels detected, dark color is the optimized output, and dashed black lines are ground truth}
\label{fig:simulated_sequence}
\end{figure}

  \begin{figure}[!h]
\centering
\begin{tabular}{cc}
    \includegraphics[width=0.45\columnwidth]
    
    &
     \includegraphics[width=0.45\columnwidth]{images/experiment/performance/depth/measure.jpg}
    \\
    \footnotesize (a)  & \footnotesize (b) \\
\end{tabular}
\caption{\textbf {Raw measures of a frame.} (a) All objects detected by the target localization module. (b) Focus map detected by the focus detection measure. White areas are focused, and black areas are out of focus. }
\label{fig:raw_measures}
\end{figure}

 \begin{figure}[!h]
\centering
\begin{tabular}{cc}   
    \includegraphics[width=0.48\columnwidth]{images/experiment/performance/pixels/opt.jpg} 
    &
     \includegraphics[width=0.48\columnwidth]{images/experiment/performance/pixels/plot_bb_gt.jpg}
    \\
    
     \footnotesize (a)  & \footnotesize (d) 
     \\
     
    \includegraphics[width=0.48\columnwidth]{images/experiment/performance/pixels/no_opt.jpg} 
    &
     \includegraphics[width=0.48\columnwidth]{images/experiment/performance/pixels/plot_only_measure.jpg}
    \\
     \footnotesize (b)  & \footnotesize (e) 
    \\
      \includegraphics[width=0.48\columnwidth]{images/experiment/performance/depth/gt.jpg} 
    &
     \includegraphics[width=0.48\columnwidth]{images/experiment/performance/depth/plot_measure_opt.jpg}
   \\
     \footnotesize (c)  & \footnotesize (f) \\
\end{tabular}
\caption{\textbf {Analysis of the features of a frame from a real sequence.} %Measures and optimized output of the target detection module and focus detection module.
(a) Optimized output of the target localization module, with only one main target selected. Green box is ground truth and the red box is optimized output. (b) Wrong selection of the main target if the continuity between frames is not taken into account in the optimization problem. (c) Optimized output of the focus detection module. Target and Foreground are out of focus, background is in focus. (d) Optimized Bounding box of the target localization module. Light colors are ground truth and dark colors are the output. Blue lines are horizontal components and orange are vertical components (e) Not Optimized Bounding box of the target localization module. Note the misdetection in some frames compared to the ground truth values (f) Optimized output of blurry module (dark colors) together with the blurry measures in percentage (light colors). Yellow is background, orange is foregound and blue is target. %Light colors represent the measures and dark colors represent the optimized output. 
1 is focused and 0 is not focused.}
\label{fig:real_sequence}
\end{figure}



  \subsection{Quality of style features extracted}
\label{sec:sequence-analyze}
   %Another sequence here?
The goal of this experiment is to measure the quality of the features extracted to encode the input sequences style.
%demonstrate that this algorithm extracts the correct features from the input sequence, we validate the quality of 
We analyze
the localization of the image position and body joints of the main targets, as well as the focus of the different image regions. 

%With that aim, we use 
To have the ground truth values for these magnitudes, this experiment uses an input sequence generated in the photorealistic environment XXXX????. 

and we manually tag each frame of the real sequence with the bounding box that localizes the main target in the image and the focus of the scene. 

%Then, the values of the output of the pipeline are compared with the ground truth values in both sequences.

% Then, we perform a similar comparison of the focus, comparing tagged values with the optimized values from this solution.

%, and the focus of the scene -if the foreground, background, and target appear in focus in the image-. We then compare the values of the output with the ground truth value. Moreover, we show the potential of the optimization of the outputs by comparing the outputs of the measures not optimized with the ground truth value.
\subsubsection{Results of target and body joints localization}
%Figure \ref{fig:performance-qualitative} shows qualitative results for a determinate frame of the sequence. 
%With respect to target localization, 
 Figure~\ref{fig:raw_measures}-a depicts all the objects detected by Mask-RCNN in this frame of the real sequence. Among all the objects, three are identified as 'person' and only the main target should be selected. %CineTransfer filters and optimizes the results, localizing the target on the image  from the noisy measurement. % but only the main target should be selected.  
 Figure \ref{fig:real_sequence}-a shows the bounding box of the selected main target  in red and its ground truth in green. For quantitative results, we refer the reader to Fig. \ref{fig:real_sequence}-d, which shows 
the four components of the optimized bounding box over the frames and its ground truth. Dark and light  blue represent the horizontal ($x$) components and their ground truth, respectively.
 Analogously, dark and light orange lines represent the vertical ($y$) components. Note that the optimized values are close to the ground-truth values despite the noisy measurements, proving the correct localization of the main target.
The body joints localization performance is demonstrated by comparing the output of CineTransfer with the ground truth values of the simulated sequence. For qualitative results, Fig.\ref{fig:simulated_sequence}-a,b show two frames of the sequence with the detected skeleton. For quantitative results, Fig.\ref{fig:simulated_sequence}-d shows the 2D point of the image ($x$ is blue and $y$ is orange),, normalized from 0 to 1, where the chest of the person  (red middle point in the graphical skeleton) is localized and optimized by CineTransfer over frames. Dashed lines represent ground-truth values and solid lines represent the output of the algorithm.

\subsubsection{Results of focus}
% This example shows how the optimization problem reduces the noise of the measure and predicts the correct output based on the continuity of the frames. 
The raw output of EFENet for the frames analyzed is depicted in  Fig.\ref{fig:simulated_sequence}-c for the simulated sequence and in Fig.\ref{fig:raw_measures}-b  for the real sequence.
Light areas represent the part of the scene that is in focus and dark parts are out of focus.
In the frame of the simulated sequence, the main target is the only part that is shown in focus, so the foreground and background remain out of focus. 
For quantitative results, Fig.\ref{fig:simulated_sequence}-f depicts the comparison of the percentage of focused pixels of the target optimized (dark colors) together with the raw noisy measures from the library (light color), and the ground truth values (black dashed line, 1 is focused, 0 is not focused) over frames. %Yellow, orange, and blue lines represent the focus of the background, foreground, and target, respectively. 
In the frame of the real sequence, the background is the only part that is shown in focus, so the foreground and main target remain out of focus.
Figure \ref{fig:real_sequence}-c depicts a graphical representation of the  focus of this frame optimized, which matches the ground truth value. For quantitative results, Fig.\ref{fig:real_sequence}-f depicts the comparison of the percentage of focused pixels optimized (dark colors) together with the raw noisy measures from the library (light colors) over frames. Yellow, orange, and blue lines represent the focus of the background, foreground, and target, respectively. 



%The output of EFENet extracts a boolean map that represents the pixels that are in/out of focus in a picture, which is depicted in Fig.\ref{fig:raw_measures}-b for this frame. Light areas represent the part of the scene that is in focus and dark parts are out of focus.
%In this frame, the background is the only part that is shown in focus, so the foreground and main target remain out of focus. Fig.\ref{fig:performance-qualitative}-e depicts a graphical representation of the output of CineTransfer, once optimized, which matches with the ground truth value. For quantitative results, Fig.\ref{fig:performance-qualitative}-f depicts the comparison of the percentage of focused pixels optimized (dark colors) together with the raw noisy measures from the library (light colors). Yellow, orange, and blue lines represent the focus of the background, foreground, and target, respectively. 
%Analogously, Fig.\ref{fig:performance-qualitative}d represents the evolution of the output only by taking into account the measures.


%Fig.\ref{fig:performance-qualitative}e. Figure \ref{fig:performance-quantitative}a depicts a graphical representation of the evolution of the optimized bounding box of the target along the frames of the sequence. Light blue and dark blue represent the ground truth values of the vertical components of the bounding box and the output of the optimization, respectively. Analogously, light and dark orange lines represent the horizontal components of the bounding box.

\subsubsection{The importance of the continuity term}
In this experiment, we prove how the optimization problem helps to improve the final output. %extract the output of the library if the 
In the first test, we analyze again the real sequence, but the cost term, which guarantees the continuity of the output of the bounding box of the main target ($\Theta_{f,t}$ of Eq. \ref{eq:cost-pixels}), is deactivated. Consequently, the bounding box of the main target is localized by only using the measure of the library,
\begin{equation}
\begin{aligned}
\min_{\substack{\mathbf{R}_{f,t}\\{\alpha_{f,t}}}} \quad & \sum_{f=0}^{nf}\sum_{t=0}^{nt}{\sum_{m=0}^{nm}\Pi_{f,t,m} }\\
\textrm{s.t.}
%\quad & 0 < BB_{f,t}.height < f.height \\  
%& 0 < BB_{f,t}.width < f.width  \\
 \quad & \mathbf{R}_{f,t} \in f \\
& \sum_{m=0}^{nm}{\alpha_{f,m}} = 1,  \ 0 < \alpha_{f,m}< 1 
\end{aligned}.
\end{equation}
% by setting. $w_cont$ to zero. 

Figure \ref{fig:real_sequence}-b shows the detected bounding box (red), and the expected ground truth value (green) for the analyzed frame. The optimization problem incorrectly selects the bounding box of a person that is not the main target. This might be caused because the main target appears blurry, which impacts negatively the confidence on the measure of that mask, $q_{f,m}$. The selected person appears in focus, having higher confidence, % as it appears in focus, 
and misleading to a wrong detection. %Analogously to the optimized detection, 
Figure \ref{fig:real_sequence}-e shows the components of the bounding box over the frames when only the measure of the library is used. Note how the main target is not localized correctly from frame 20 to frame 40.

Analogously, we analyze again the simulated sequence but this time, we deactivate the cost term that ensures the continuity of output of the body joints of the target over frames. In this sequence, the target is moving, so the position of the body joints varies significantly from one frame to another. Figures \ref{fig:simulated_sequence}-a and \ref{fig:simulated_sequence}-b represent this variation in two subsequent frames. The optimization problem helps to reduce this noise, providing a continuous output for a more stable framing of the target. Figure \ref{fig:simulated_sequence}-e shows the vertical component of the chest optimized (dark blue) and not optimized (light blue) normalized from 0 to 1.
Note how the optimized output is softer, reducing the noise induced by the movement of the target.



%  \begin{figure}[!h]
% \centering
% \begin{tabular}{cc}
 
%     \includegraphics[width=0.48\columnwidth]{images/experiment/performance/pixels/plot_bb_gt.jpg} 
%     &
%      \includegraphics[width=0.48\columnwidth]{images/experiment/performance/depth/plot_measure_opt.jpg}
%    \\
    
%      \footnotesize (a)  & \footnotesize (c) \\
%     \\
%        \includegraphics[width=0.48\columnwidth]{images/experiment/performance/pixels/plot_only_measure.jpg} 
%     &
%      \includegraphics[width=0.48\columnwidth]{images/4.png} \\
%      \footnotesize (b)  & \footnotesize (d) \\
% \end{tabular}
% \caption{\textbf {Quantitative experiments}- (d) ? }
% \label{fig:performance-quantitative}
% \end{figure}

  

\begin{figure*}[!th]
\centering
\begin{tabular}{cccc}
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/original/1.jpg} 
    &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/copy/1.jpg} 
    &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/footbal/1.jpg} 
    &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Quantitative/1.jpg} 
    \\
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/original/3.jpg} 
    &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/copy/3.jpg} 
    &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/footbal/3.jpg}  &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Quantitative/2.jpg} 
    \\
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/original/4_open.jpg} 
    &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/copy/4_open.jpg} 
    &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/footbal/4_open.jpg}  &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Quantitative/3.jpg} 
    \\

    \footnotesize (a)  & \footnotesize (b) & \footnotesize (c)  & \footnotesize (d)  \\
\end{tabular}
\caption{\textbf {Comparison - Qualitative experiments}}
\label{fig:exp_comparing}
\end{figure*}

  \subsection{Style Transfer examples from real sequences}
This experiment demonstrates how CineTransfer extracts the main features of an input sequence and gives instructions to a cinematographic platform to recreate the sequence in a similar and a different scenario. Concretely, we use CineMPC  \cite{pueyo2022cinempc}, a cinematographic platform that receives recording instructions, i.e. desired depth of field, desired position of targets in the scene, and solves an MPC optimization problem to move a drone and a camera satisfying the given instructions. We adapted CineMPC to read the CineTransfer JSON files and use them as recording instructions.
In this experiment, we reproduce the input sequence that has been analyzed in Sec. \ref{sec:sequence-analyze} in the photorealistic simulator CinemAirSim\cite{pueyo2020cinemairsim}, an extension of AirSim \cite{shah2018airsim} for cinematographic purposes. The sequence is first reproduced in a scenario similar to the input sequence, showing the artistic and purely aesthetic output of this solution for qualitative comparison between the two sequences. In the second experiment, the sequence is reproduced in a scenario that is very different from the input sequence %, but there is a main target in the scene 
for qualitative and quantitative results by comparing the output of CineTransfer in both the input and output sequences.

%is able to extract the features of a scene, independently of the scene or the scenario where the sequence is recorded.

%The idea of CineTransfer is to move a drone to recreate the features of a scene, independently of the scene or the scenario where the sequence is recorded. In this subsection, we use CineMPC\cite{pueyo2022cinempc} to obtain two output sequences in different scenarios by using the same input sequence. 

%It is important to remark, that in that solution, the localization of the targets in the scene is given for granted. First, we perform experiments in a scenario that is very similar to the one where the input sequence was recorded and compare the two sequences qualitatively, showing the artistic and purely aesthetic output of our solution. Then, we use a scenario, where there is a target, that is very different from the input sequence. In this case, we obtain qualitative and quantitative results by comparing the output of CineTransfer for both the input and output sequences.
% Salidas de blurry y de bounding box optimizando con GT
% Selección del target de interes. Mostrar qué pasa si no se optimiza, o si se desactiva el termino de continuidad. Destacar que en esta sequencia aparece mucha gente por detrás que genera ruido
% Comparar blurry con GT optimizando y sin optimizar 


  \subsubsection{Qualitative experiments}
 %The first three columns of Fig. \ref{fig:exp_comparing} depict different frames of the experiment  
 The target position on the image and the focus of the scene vary along the sequence. The first three columns of Fig. \ref{fig:exp_comparing} depict three frames of the beginning, middle, and end of the sequence ordered top to bottom in time for qualitative comparison.
 First column depicts the frames of the input sequence%(from the movie Road to Perdition), 
, second column represents the same frames from the cloned sequence in a similar scenario and the third column shows the same frames recorded in a scenario that is different (football player standing up in the mountains). The frames on the bottom include a graphical representation of the points of interest of the main target for comparison. At the beginning of the sequence (first row), the main target is placed in the center and showing in focus, in the middle (second row) the target appears closer in the image and out of focus, and at the end of the sequence (third row) the target appears much closer and in focus, showing the background out of focus. Note how the cloned scenes (second and third columns) reproduce these effects qualitatively. 
  
  
  %The qualitative experiments are depicted in the three first columns of Fig. \ref{fig:exp_comparing}. The first column represents some frames from the input sequence. The second column represents the same frames from the output sequence in the scenario that is similar to the one where the input sequence is recorded. The same frames recorded in the scenario that is different (football player standing up in the mountains) are depicted in the third column. As a guideline, the bottom frames include the output of OpenPose.

  \subsubsection{Quantitative experiments}
Different plots are shown in the fourth column of Fig.~\ref{fig:exp_comparing} for quantitative comparison between the input sequence (first column) and the sequence cloned in a different scenario (third column). Both sequences are analyzed by CineTransfer to compare the results of the outputs. The results are shown in the plots, where light colors represent the values on the input sequence and dark colors represent the values on the cloned sequence. The comparison of the focus of the two sequences over frames is depicted in the first row. Yellow, orange, and blue lines represent the background, foreground, and target, respectively.
The second row represents the pixels of the bounding box of the target localized in the input sequence and the same output in the output sequence. Blue lines are vertical components and orange lines are horizontal components. Lastly, the bottom row represents the evolution of the vertical (orange) and horizontal (blue) positions of the left and right shoulders which are the parts of the body that are controlled to frame the target in this experiment. Note that the values shown in the last two rows are normalized by dividing the image position by the image height/width to support different image sensor sizes.


  
%To show the artistic and purely aesthetic output of our solution, we have recreated the scenario of the input sequence. The main target appears sitting  down at the end of a table while the focus and position of the target on the image are continuously changing. 
%Fig. shows the comparison of some frames of the real sequence from the real movie, with the recreated scene using CineMPC.

%  \begin{figure}[!h]
% \centering
% \begin{tabular}{cc}
%     \includegraphics[width=0.40\columnwidth]{images/experiment/Qualitative/copy/frame9.jpg} 
%     &
%      \includegraphics[width=0.53\columnwidth]{images/experiment/Qualitative/original/frame1.jpg}
%     \\
%     \includegraphics[width=0.40\columnwidth]{images/experiment/Qualitative/copy/frame18.jpg} 
%     &
%      \includegraphics[width=0.53\columnwidth]{images/experiment/Qualitative/original/frame20.jpg}
%     \\
%     \includegraphics[width=0.40\columnwidth]{images/experiment/Qualitative/copy/frame35.jpg} 
%     &
%      \includegraphics[width=0.53\columnwidth]{images/experiment/Qualitative/original/frame35.jpg}
%     \\
%     \includegraphics[width=0.40\columnwidth]{images/experiment/Qualitative/copy/frame47.jpg} 
%     &
%      \includegraphics[width=0.53\columnwidth]{images/experiment/Qualitative/original/frame47.jpg}
%     \\
%     \footnotesize (c) Body joints of targets & \footnotesize (d) Masks and BB of targets \\
% \end{tabular}
% \caption{\textbf {Comparison - Qualitative experiments}}
% \label{fig:measures}
% \end{figure}

% \subsection{Comparison - Quantitative experiments}





























































% \red{To show the potential of our solution, we present a complete cinematographic recording composed by seven parts. Each part 
% demonstrates different artistic requirements or specifications that CineMPC helps to fulfill.
% %transmit different emotional and artistic sensations. 
% Next we describe the implementation and execution details and discuss the experiment content and analysis.

% \subsection{Implementation details}
% The system is implemented in C++ and communicates with CinemAirSim \cite{pueyo2020cinemairsim}. Thus, this work is validated in a photorealistic scenario where drones have realistic physics and dynamics. AirSim implements a low-level controller for the drone that takes a trajectory of 3D world points and a desired velocity as input and moves the drone accordingly. CineMPC calculates a set of 3D points and velocities according to the actuators that this low-level controller transforms into a feasible trajectory and gives the commands to the drone.
% %Additionally, more sophisticated trajectories can be handled by existing trajectory optimizations like \cite{richter2016polynomial}, which outputs a polynomial high-quality trajectory of the position and its different derivatives.
% Since the proposed optimization problem is non-linear, we use Ipopt (Interior Point OPTimizer) \cite{wachter2006implementation} to solve the MPC problem.
% The ground-truth data used for the experiments is obtained from AirSim. In order to make experiments closer to reality, i.e. to simulate more realistic measures, the provided position of the targets is perturbed with a Gaussian noise of zero mean and standard deviation of $\sigma = 0.04m^2,$ for each component. Based on experimentation and knowledge, a Gaussian noise with these values introduces a reasonable perturbation that the system can absorb without lowering its performance.  The orientation of the targets is perturbed with a Gaussian noise of zero mean and standard deviation of $\sigma = 0.01$rad$^2$.  These noisy measures are filtered with a Kalman Filter in order to reduce the noise impact in the final result, as we would do in real world scenarios. The filter would also be useful for robust estimation of the pose of the targets in case of a miss-detection in a real case scenario. 
% %\red{add figure of stimations? Look at fig 2 [3,e]}

% The system is composed of different modules. One module is in charge of reading the state of the system, another module runs the MPC according to this state and user's instructions and calculates the next $N$ discrete steps, a third module joints these steps creating a more continuous and softer spline trajectory that gives to the drone. Each module is run in a different thread, the main thread handles the communication and synchronization between them. %The implementation will be released .... ???  
% %which adds an extra level of complexity due to the communication and synchronization between them.%In this section, we demonstrate CineTransfer's capacity to analyze two input sequences, one from a simulation where we know the ground truth values, and another one from a real movie. Then, we validate the solution using an existing cinematographic drone controller to recreate the real scene in photorealistic simulation.

This section validates CineTransfer's capabilities to \textit{transfer} the style of different input sequences to new automatically acquired recordings in a photo-realistic virtual environment.

The input sequences chosen cover the main aspects to be validated: XXXX (sequence ?), XXXX (sequence ?) and XXXX (sequence ?). This last input sequence is generated in a virtual environment to facilitate quantitative evaluation of ??.

\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c}
                      & Input seq. & Output seq. &  Focus & Main target & Body joints & Target framing \\
         E1 & Sim. & Sim. & TICK & CROSS & \\
         E2 & Real & Sim. \\
         %Experiment 3 & Real & Photorealistic \\
         %Experiment 4 & Real & Photorealistic \\
         
    \end{tabular}
    \caption{Experimental validation}
    \label{tab:my_label}
\end{table}


%The very end of CineTransfer is to control a cinematographic platform by using an input sequence as recording instructions, easing its introduction to users that are not experts. 
%To demonstrate its potential, we present a full experiment whose objective is to reproduce a 

For the simulated sequence, we have recorded a fireman walking in the mountains. In this sequence, the focus of the target changes, and the target is walking, which causes the measures of the body's keypoints be noisy. The sequence is divided into 99 frames that are captured every 0.5 s.
For the real sequence, we have chosen a sequence of 25 s. from the movie "Road to Perdition", awarded the Oscars for best photography in 2003. This sequence is particularly challenging because multiple persons and objects appear, but only one of them is the main target, and there are changes in the depth of field. The sequence is divided into 48 frames that are captured every 0.5 s.

We perform different qualitative and quantitative experiments to demonstrate the capacity of the solution, and we refer the reader to the supplementary video for more complete visual results.


%First, we show how the two sequences are analyzed and the features of the sequence, appropriately optimized. Then, we transform the features into constraints of CineMPC as defined in Sec. \ref{sec_problem_formulation} to recreate the sequence in two different scenarios, and analyze the results.

 \subsection{Implementation details}
 All the experiments are run in Ubuntu 20 on an AMD Ryzen 9 5900X 12-Core CPU equipped with 32 Gb of RAM and an NVidia GeForce GTX 3090 Ti. The pipeline of CineTransfer is implemented in Python. It makes calls to the libraries to detect the focus, the mask, and the position of the targets of the image and collects and optimizes the results, using the Python optimization library Gekko \cite{gekko}, and generate the JSON files. Then, have modified CineMPC which is implemented in ROS and C++ to read the recording instructions from the JSON files.
 
 
 \begin{figure}[!h]
\centering
\begin{tabular}{cc}
    \includegraphics[width=0.48\columnwidth,height=2.1cm]{images/experiment2/pose_1.jpg} 
    &
    
     \includegraphics[width=0.48\columnwidth]{images/experiment2/keypoint.jpg}
    \\ 
    
    \footnotesize (a)  & \footnotesize (d) \\
    
    \includegraphics[width=0.48\columnwidth,height=2.1cm]{images/experiment2/pose_2.jpg} 
    &
    \includegraphics[width=0.48\columnwidth]{images/experiment2/noisy.jpg}
    \\
     \footnotesize (b)  & \footnotesize (e) \\
     
    \includegraphics[width=0.48\columnwidth,height=2.1cm]{images/experiment2/frame0.jpg} 
    &
     \includegraphics[width=0.48\columnwidth]{images/experiment2/focus.jpg}
    \\
     \footnotesize (c)  & \footnotesize (f) \\
\end{tabular}
\caption{\textbf {Analysis of the features of a frame from a simulated sequence.}(a-b) Two subsequent frames of the sequence showing the skeleton for the body joints detection algorithm (c) Focus map detected by the focus detection measure. White areas are focused, and black areas are out of focus. (d) Plot showing the ground truth (light color) and CineTransfer values for the point of the chest of the target (red middle point in skeleton). Blue are vertical components and Orange are horizontal components (e) Vertical component of the chest of the target when the continuity between frames is not optimized (light) and when it is (dark) (f) Evolution of the detected focus of the main target. Light color is the percentage of pixels detected, dark color is the optimized output, and dashed black lines are ground truth}
\label{fig:simulated_sequence}
\end{figure}

  \begin{figure}[!h]
\centering
\begin{tabular}{cc}
    \includegraphics[width=0.45\columnwidth]{images/experiment/performance/pixels/measure.png} 
    &
     \includegraphics[width=0.45\columnwidth]{images/experiment/performance/depth/measure.jpg}
    \\
    \footnotesize (a)  & \footnotesize (b) \\
\end{tabular}
\caption{\textbf {Raw measures of a frame.} (a) All objects detected by the target localization module. (b) Focus map detected by the focus detection measure. White areas are focused, and black areas are out of focus. }
\label{fig:raw_measures}
\end{figure}

 \begin{figure}[!h]
\centering
\begin{tabular}{cc}   
    \includegraphics[width=0.48\columnwidth]{images/experiment/performance/pixels/opt.jpg} 
    &
     \includegraphics[width=0.48\columnwidth]{images/experiment/performance/pixels/plot_bb_gt.jpg}
    \\
    
     \footnotesize (a)  & \footnotesize (d) 
     \\
     
    \includegraphics[width=0.48\columnwidth]{images/experiment/performance/pixels/no_opt.jpg} 
    &
     \includegraphics[width=0.48\columnwidth]{images/experiment/performance/pixels/plot_only_measure.jpg}
    \\
     \footnotesize (b)  & \footnotesize (e) 
    \\
      \includegraphics[width=0.48\columnwidth]{images/experiment/performance/depth/gt.jpg} 
    &
     \includegraphics[width=0.48\columnwidth]{images/experiment/performance/depth/plot_measure_opt.jpg}
   \\
     \footnotesize (c)  & \footnotesize (f) \\
\end{tabular}
\caption{\textbf {Analysis of the features of a frame from a real sequence.} %Measures and optimized output of the target detection module and focus detection module.
(a) Optimized output of the target localization module, with only one main target selected. Green box is ground truth and the red box is optimized output. (b) Wrong selection of the main target if the continuity between frames is not taken into account in the optimization problem. (c) Optimized output of the focus detection module. Target and Foreground are out of focus, background is in focus. (d) Optimized Bounding box of the target localization module. Light colors are ground truth and dark colors are the output. Blue lines are horizontal components and orange are vertical components (e) Not Optimized Bounding box of the target localization module. Note the misdetection in some frames compared to the ground truth values (f) Optimized output of blurry module (dark colors) together with the blurry measures in percentage (light colors). Yellow is background, orange is foregound and blue is target. %Light colors represent the measures and dark colors represent the optimized output. 
1 is focused and 0 is not focused.}
\label{fig:real_sequence}
\end{figure}



  \subsection{Quality of style features extracted}
\label{sec:sequence-analyze}
   %Another sequence here?
The goal of this experiment is to measure the quality of the features extracted to encode the input sequences style.
%demonstrate that this algorithm extracts the correct features from the input sequence, we validate the quality of 
We analyze
the localization of the image position and body joints of the main targets, as well as the focus of the different image regions. 

%With that aim, we use 
To have the ground truth values for these magnitudes, this experiment uses an input sequence generated in the photorealistic environment XXXX????. 

and we manually tag each frame of the real sequence with the bounding box that localizes the main target in the image and the focus of the scene. 

%Then, the values of the output of the pipeline are compared with the ground truth values in both sequences.

% Then, we perform a similar comparison of the focus, comparing tagged values with the optimized values from this solution.

%, and the focus of the scene -if the foreground, background, and target appear in focus in the image-. We then compare the values of the output with the ground truth value. Moreover, we show the potential of the optimization of the outputs by comparing the outputs of the measures not optimized with the ground truth value.
\subsubsection{Results of target and body joints localization}
%Figure \ref{fig:performance-qualitative} shows qualitative results for a determinate frame of the sequence. 
%With respect to target localization, 
 Figure~\ref{fig:raw_measures}-a depicts all the objects detected by Mask-RCNN in this frame of the real sequence. Among all the objects, three are identified as 'person' and only the main target should be selected. %CineTransfer filters and optimizes the results, localizing the target on the image  from the noisy measurement. % but only the main target should be selected.  
 Figure \ref{fig:real_sequence}-a shows the bounding box of the selected main target  in red and its ground truth in green. For quantitative results, we refer the reader to Fig. \ref{fig:real_sequence}-d, which shows 
the four components of the optimized bounding box over the frames and its ground truth. Dark and light  blue represent the horizontal ($x$) components and their ground truth, respectively.
 Analogously, dark and light orange lines represent the vertical ($y$) components. Note that the optimized values are close to the ground-truth values despite the noisy measurements, proving the correct localization of the main target.
The body joints localization performance is demonstrated by comparing the output of CineTransfer with the ground truth values of the simulated sequence. For qualitative results, Fig.\ref{fig:simulated_sequence}-a,b show two frames of the sequence with the detected skeleton. For quantitative results, Fig.\ref{fig:simulated_sequence}-d shows the 2D point of the image ($x$ is blue and $y$ is orange),, normalized from 0 to 1, where the chest of the person  (red middle point in the graphical skeleton) is localized and optimized by CineTransfer over frames. Dashed lines represent ground-truth values and solid lines represent the output of the algorithm.

\subsubsection{Results of focus}
% This example shows how the optimization problem reduces the noise of the measure and predicts the correct output based on the continuity of the frames. 
The raw output of EFENet for the frames analyzed is depicted in  Fig.\ref{fig:simulated_sequence}-c for the simulated sequence and in Fig.\ref{fig:raw_measures}-b  for the real sequence.
Light areas represent the part of the scene that is in focus and dark parts are out of focus.
In the frame of the simulated sequence, the main target is the only part that is shown in focus, so the foreground and background remain out of focus. 
For quantitative results, Fig.\ref{fig:simulated_sequence}-f depicts the comparison of the percentage of focused pixels of the target optimized (dark colors) together with the raw noisy measures from the library (light color), and the ground truth values (black dashed line, 1 is focused, 0 is not focused) over frames. %Yellow, orange, and blue lines represent the focus of the background, foreground, and target, respectively. 
In the frame of the real sequence, the background is the only part that is shown in focus, so the foreground and main target remain out of focus.
Figure \ref{fig:real_sequence}-c depicts a graphical representation of the  focus of this frame optimized, which matches the ground truth value. For quantitative results, Fig.\ref{fig:real_sequence}-f depicts the comparison of the percentage of focused pixels optimized (dark colors) together with the raw noisy measures from the library (light colors) over frames. Yellow, orange, and blue lines represent the focus of the background, foreground, and target, respectively. 



%The output of EFENet extracts a boolean map that represents the pixels that are in/out of focus in a picture, which is depicted in Fig.\ref{fig:raw_measures}-b for this frame. Light areas represent the part of the scene that is in focus and dark parts are out of focus.
%In this frame, the background is the only part that is shown in focus, so the foreground and main target remain out of focus. Fig.\ref{fig:performance-qualitative}-e depicts a graphical representation of the output of CineTransfer, once optimized, which matches with the ground truth value. For quantitative results, Fig.\ref{fig:performance-qualitative}-f depicts the comparison of the percentage of focused pixels optimized (dark colors) together with the raw noisy measures from the library (light colors). Yellow, orange, and blue lines represent the focus of the background, foreground, and target, respectively. 
%Analogously, Fig.\ref{fig:performance-qualitative}d represents the evolution of the output only by taking into account the measures.


%Fig.\ref{fig:performance-qualitative}e. Figure \ref{fig:performance-quantitative}a depicts a graphical representation of the evolution of the optimized bounding box of the target along the frames of the sequence. Light blue and dark blue represent the ground truth values of the vertical components of the bounding box and the output of the optimization, respectively. Analogously, light and dark orange lines represent the horizontal components of the bounding box.

\subsubsection{The importance of the continuity term}
In this experiment, we prove how the optimization problem helps to improve the final output. %extract the output of the library if the 
In the first test, we analyze again the real sequence, but the cost term, which guarantees the continuity of the output of the bounding box of the main target ($\Theta_{f,t}$ of Eq. \ref{eq:cost-pixels}), is deactivated. Consequently, the bounding box of the main target is localized by only using the measure of the library,
\begin{equation}
\begin{aligned}
\min_{\substack{\mathbf{R}_{f,t}\\{\alpha_{f,t}}}} \quad & \sum_{f=0}^{nf}\sum_{t=0}^{nt}{\sum_{m=0}^{nm}\Pi_{f,t,m} }\\
\textrm{s.t.}
%\quad & 0 < BB_{f,t}.height < f.height \\  
%& 0 < BB_{f,t}.width < f.width  \\
 \quad & \mathbf{R}_{f,t} \in f \\
& \sum_{m=0}^{nm}{\alpha_{f,m}} = 1,  \ 0 < \alpha_{f,m}< 1 
\end{aligned}.
\end{equation}
% by setting. $w_cont$ to zero. 

Figure \ref{fig:real_sequence}-b shows the detected bounding box (red), and the expected ground truth value (green) for the analyzed frame. The optimization problem incorrectly selects the bounding box of a person that is not the main target. This might be caused because the main target appears blurry, which impacts negatively the confidence on the measure of that mask, $q_{f,m}$. The selected person appears in focus, having higher confidence, % as it appears in focus, 
and misleading to a wrong detection. %Analogously to the optimized detection, 
Figure \ref{fig:real_sequence}-e shows the components of the bounding box over the frames when only the measure of the library is used. Note how the main target is not localized correctly from frame 20 to frame 40.

Analogously, we analyze again the simulated sequence but this time, we deactivate the cost term that ensures the continuity of output of the body joints of the target over frames. In this sequence, the target is moving, so the position of the body joints varies significantly from one frame to another. Figures \ref{fig:simulated_sequence}-a and \ref{fig:simulated_sequence}-b represent this variation in two subsequent frames. The optimization problem helps to reduce this noise, providing a continuous output for a more stable framing of the target. Figure \ref{fig:simulated_sequence}-e shows the vertical component of the chest optimized (dark blue) and not optimized (light blue) normalized from 0 to 1.
Note how the optimized output is softer, reducing the noise induced by the movement of the target.



%  \begin{figure}[!h]
% \centering
% \begin{tabular}{cc}
 
%     \includegraphics[width=0.48\columnwidth]{images/experiment/performance/pixels/plot_bb_gt.jpg} 
%     &
%      \includegraphics[width=0.48\columnwidth]{images/experiment/performance/depth/plot_measure_opt.jpg}
%    \\
    
%      \footnotesize (a)  & \footnotesize (c) \\
%     \\
%        \includegraphics[width=0.48\columnwidth]{images/experiment/performance/pixels/plot_only_measure.jpg} 
%     &
%      \includegraphics[width=0.48\columnwidth]{images/4.png} \\
%      \footnotesize (b)  & \footnotesize (d) \\
% \end{tabular}
% \caption{\textbf {Quantitative experiments}- (d) ? }
% \label{fig:performance-quantitative}
% \end{figure}

  

\begin{figure*}[!th]
\centering
\begin{tabular}{cccc}
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/original/1.jpg} 
    &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/copy/1.jpg} 
    &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/footbal/1.jpg} 
    &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Quantitative/1.jpg} 
    \\
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/original/3.jpg} 
    &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/copy/3.jpg} 
    &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/footbal/3.jpg}  &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Quantitative/2.jpg} 
    \\
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/original/4_open.jpg} 
    &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/copy/4_open.jpg} 
    &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/footbal/4_open.jpg}  &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Quantitative/3.jpg} 
    \\

    \footnotesize (a)  & \footnotesize (b) & \footnotesize (c)  & \footnotesize (d)  \\
\end{tabular}
\caption{\textbf {Comparison - Qualitative experiments}}
\label{fig:exp_comparing}
\end{figure*}

  \subsection{Style Transfer examples from real sequences}
This experiment demonstrates how CineTransfer extracts the main features of an input sequence and gives instructions to a cinematographic platform to recreate the sequence in a similar and a different scenario. Concretely, we use CineMPC  \cite{pueyo2022cinempc}, a cinematographic platform that receives recording instructions, i.e. desired depth of field, desired position of targets in the scene, and solves an MPC optimization problem to move a drone and a camera satisfying the given instructions. We adapted CineMPC to read the CineTransfer JSON files and use them as recording instructions.
In this experiment, we reproduce the input sequence that has been analyzed in Sec. \ref{sec:sequence-analyze} in the photorealistic simulator CinemAirSim\cite{pueyo2020cinemairsim}, an extension of AirSim \cite{shah2018airsim} for cinematographic purposes. The sequence is first reproduced in a scenario similar to the input sequence, showing the artistic and purely aesthetic output of this solution for qualitative comparison between the two sequences. In the second experiment, the sequence is reproduced in a scenario that is very different from the input sequence %, but there is a main target in the scene 
for qualitative and quantitative results by comparing the output of CineTransfer in both the input and output sequences.

%is able to extract the features of a scene, independently of the scene or the scenario where the sequence is recorded.

%The idea of CineTransfer is to move a drone to recreate the features of a scene, independently of the scene or the scenario where the sequence is recorded. In this subsection, we use CineMPC\cite{pueyo2022cinempc} to obtain two output sequences in different scenarios by using the same input sequence. 

%It is important to remark, that in that solution, the localization of the targets in the scene is given for granted. First, we perform experiments in a scenario that is very similar to the one where the input sequence was recorded and compare the two sequences qualitatively, showing the artistic and purely aesthetic output of our solution. Then, we use a scenario, where there is a target, that is very different from the input sequence. In this case, we obtain qualitative and quantitative results by comparing the output of CineTransfer for both the input and output sequences.
% Salidas de blurry y de bounding box optimizando con GT
% Selección del target de interes. Mostrar qué pasa si no se optimiza, o si se desactiva el termino de continuidad. Destacar que en esta sequencia aparece mucha gente por detrás que genera ruido
% Comparar blurry con GT optimizando y sin optimizar 


  \subsubsection{Qualitative experiments}
 %The first three columns of Fig. \ref{fig:exp_comparing} depict different frames of the experiment  
 The target position on the image and the focus of the scene vary along the sequence. The first three columns of Fig. \ref{fig:exp_comparing} depict three frames of the beginning, middle, and end of the sequence ordered top to bottom in time for qualitative comparison.
 First column depicts the frames of the input sequence%(from the movie Road to Perdition), 
, second column represents the same frames from the cloned sequence in a similar scenario and the third column shows the same frames recorded in a scenario that is different (football player standing up in the mountains). The frames on the bottom include a graphical representation of the points of interest of the main target for comparison. At the beginning of the sequence (first row), the main target is placed in the center and showing in focus, in the middle (second row) the target appears closer in the image and out of focus, and at the end of the sequence (third row) the target appears much closer and in focus, showing the background out of focus. Note how the cloned scenes (second and third columns) reproduce these effects qualitatively. 
  
  
  %The qualitative experiments are depicted in the three first columns of Fig. \ref{fig:exp_comparing}. The first column represents some frames from the input sequence. The second column represents the same frames from the output sequence in the scenario that is similar to the one where the input sequence is recorded. The same frames recorded in the scenario that is different (football player standing up in the mountains) are depicted in the third column. As a guideline, the bottom frames include the output of OpenPose.

  \subsubsection{Quantitative experiments}
Different plots are shown in the fourth column of Fig.~\ref{fig:exp_comparing} for quantitative comparison between the input sequence (first column) and the sequence cloned in a different scenario (third column). Both sequences are analyzed by CineTransfer to compare the results of the outputs. The results are shown in the plots, where light colors represent the values on the input sequence and dark colors represent the values on the cloned sequence. The comparison of the focus of the two sequences over frames is depicted in the first row. Yellow, orange, and blue lines represent the background, foreground, and target, respectively.
The second row represents the pixels of the bounding box of the target localized in the input sequence and the same output in the output sequence. Blue lines are vertical components and orange lines are horizontal components. Lastly, the bottom row represents the evolution of the vertical (orange) and horizontal (blue) positions of the left and right shoulders which are the parts of the body that are controlled to frame the target in this experiment. Note that the values shown in the last two rows are normalized by dividing the image position by the image height/width to support different image sensor sizes.




==> 95C_Experiments.tex <==
%In this section, we demonstrate CineTransfer's capacity to analyze two input sequences, one from a simulation where we know the ground truth values, and another one from a real movie. Then, we validate the solution using an existing cinematographic drone controller to recreate the real scene in photorealistic simulation.

This section validates CineTransfer's capabilities to \textit{transfer} the style of different input sequences to new automatically acquired recordings in a photo-realistic virtual environment.

The input sequences were chosen to cover the main aspects to be validated. The input in the first experiment is a sequence from a real movie. In this experiment, we analyze the performance of the algorithm detecting the style of the sequence: the focus, which is changing along the sequence, and the position of the main targets when more targets are present. The extracted style is then transferred to a sequence recorded in simulation.
The input of the second experiment is a sequence recorded in simulation, so we have all the ground data to facilitate quantitative evaluation of the results. In this sequence, the position of the body joints of the target is noisy and the focus of the main target varies. The style of the sequence is reproduced in simulation too.

We perform different qualitative and quantitative experiments to demonstrate the capacity of the solution, and we refer the reader to the supplementary video for more complete visual results.
%along the sequence. , so we have all the ground truth data about the focus and the position of the target and its body joints to facilitate quantitative evaluation of the results. 




% sequence 1 XXXX (sequence ?), XXXX (sequence ?) and XXXX (sequence ?). This last input sequence is generated in a virtual environment to facilitate quantitative evaluation of ??.

% \begin{table}[h]
%     \centering
%     \begin{tabular}{c|c|c|c|c|c|c}
%                       & Input seq. & Output seq. &  Focus & Main target & Body joints & Target framing \\
%          E1 & Sim. & Sim. & TICK & CROSS & \\
%          E2 & Real & Sim. \\
%          %Experiment 3 & Real & Photorealistic \\
%          %Experiment 4 & Real & Photorealistic \\
         
%     \end{tabular}
%     \caption{Experimental validation}
%     \label{tab:my_label}
% \end{table}


%The very end of CineTransfer is to control a cinematographic platform by using an input sequence as recording instructions, easing its introduction to users that are not experts. 
%To demonstrate its potential, we present a full experiment whose objective is to reproduce a 



% For the simulated sequence, we have recorded a fireman walking in the mountains. In this sequence, the focus of the target changes, and the target is walking, which causes the measures of the body's keypoints be noisy. The sequence is divided into 99 frames that are captured every 0.5 s.
% For the real sequence, we have chosen a sequence of 25 s. from the movie "Road to Perdition", awarded the Oscars for best photography in 2003. This sequence is particularly challenging because multiple persons and objects appear, but only one of them is the main target, and there are changes in the depth of field. The sequence is divided into 48 frames that are captured every 0.5 s.

% We perform different qualitative and quantitative experiments to demonstrate the capacity of the solution, and we refer the reader to the supplementary video for more complete visual results.


%First, we show how the two sequences are analyzed and the features of the sequence, appropriately optimized. Then, we transform the features into constraints of CineMPC as defined in Sec. \ref{sec_problem_formulation} to recreate the sequence in two different scenarios, and analyze the results.

 \subsection{Implementation details}
 All the experiments are run in Ubuntu 20 on an AMD Ryzen 9 5900X 12-Core CPU equipped with 32 Gb of RAM and an NVidia GeForce GTX 3090 Ti. The pipeline of CineTransfer is implemented in Python. It makes calls to the libraries to detect the focus, the mask, and the position of the targets of the image and collects and optimizes the results, using the Python optimization library Gekko \cite{gekko}, and generate the JSON files. Then, we have modified CineMPC which is implemented in ROS and C++ to read the recording instructions from the JSON files.

 
 \subsection{Experiment 1. Detecting the main targets and transferring the input style. }
 
The input of this experiment is a sequence of 25 s. from the movie "Road to Perdition", awarded with the Oscar for best photography in 2003. The sequence is particularly challenging because there are multiple changes in the focus of the scene, and
multiple persons and objects appear, but only one of them is the main target. The sequence is divided into 48 frames that are captured every 0.5 s.

  \begin{figure}[!h]
\centering
\begin{tabular}{cc}
    \includegraphics[width=0.45\columnwidth]{images/experiment/performance/pixels/measure.png} 
    &
     \includegraphics[width=0.45\columnwidth]{images/experiment/performance/depth/measure.jpg}
    \\
    \footnotesize (a)  & \footnotesize (b) \\
\end{tabular}
\caption{\textbf {Raw measures of a frame.} (a) All objects detected by the target localization module. (b) Focus map detected by the focus detection measure. White areas are focused, and black areas are out of focus. }
\label{fig:raw_measures}
\end{figure}

  \subsubsection{Quality of style features extracted}
 To measure the quality of the features extracted to encode the input sequences style, we compare
the localization of the image position of the main target, as well as the focus of the different image regions. For this comparison, we manually tag each frame of the real sequence with the bounding box that localizes the main target in the image and the focus of the scene. 

\paragraph{\textbf{{Results of target and body joints localization}}}
%Figure \ref{fig:performance-qualitative} shows qualitative results for a determinate frame of the sequence. 
%With respect to target localization, 
 Figure~\ref{fig:raw_measures}-a depicts the noisy output of Mask-RCNN in this frame. Among all the found objects, three are identified as 'person' and only the main target should be selected by CineTransfer. 
 Figure \ref{fig:real_sequence}-a shows the bounding box of the selected main target in red and its ground truth in green. For quantitative results, we refer the reader to Fig. \ref{fig:real_sequence}-d, which shows 
the four components of the optimized bounding box over the frames and its ground truth. Dark and light  blue represent the horizontal ($x$) components and their ground truth, respectively.  Analogously, dark and light orange lines represent the vertical ($y$) components. 
Note that the optimized values are close to the ground-truth values despite the noisy measurements, proving the correct localization of the main target.

 \paragraph{\textbf{Results on the focus of the scene}}
  The raw output of EFENet of one frame is depicted in Fig.\ref{fig:raw_measures}-b. Light areas represent the part of the scene that is in focus and dark parts are out of focus. In this frame, the background is the only part that is shown in focus, and the foreground and main target remain out of focus. Figure \ref{fig:real_sequence}-c depicts a graphical representation of the  focus of this frame optimized, which matches the ground truth value. For quantitative results, Fig.\ref{fig:real_sequence}-f depicts the comparison of the percentage of focused pixels optimized (dark colors) together with the raw noisy measures from the library (light colors) over frames. Orange, yellow, and blue lines represent the focus of the background, target, and foreground, respectively. 

 \paragraph{\textbf{The importance of the optimization algorithm}}
 In this section, we prove how the optimization problem helps to improve the final output. We analyze again the real sequence again, but the cost term, which guarantees the continuity of the output of the bounding box of the main target ($\Theta_{f,t}$ of Eq. \ref{eq:cost-pixels}), is deactivated. Consequently, the bounding box of the main target is localized by only using the measure of the library,
\begin{equation}
\begin{aligned}
\min_{\substack{\mathbf{R}_{f,t}\\{\alpha_{f,t}}}} \quad & \sum_{f=0}^{nf}\sum_{t=0}^{nt}{\sum_{m=0}^{nm}\Pi_{f,t,m} }\\
\textrm{s.t.}
%\quad & 0 < BB_{f,t}.height < f.height \\  
%& 0 < BB_{f,t}.width < f.width  \\
 \quad & \mathbf{R}_{f,t} \in f \\
& \sum_{m=0}^{nm}{\alpha_{f,m}} = 1,  \ 0 < \alpha_{f,m}< 1 
\end{aligned}.
\end{equation}

Figure \ref{fig:real_sequence}-b shows the detected bounding box (red), and the expected ground truth value (green) for the analyzed frame. The optimization problem incorrectly selects the bounding box of a person that is not the main target. This might be caused because the main target appears blurry, which impacts negatively the confidence on the measure of that mask, $q_{f,m}$. The selected person appears in focus, having higher confidence, % as it appears in focus, 
and misleading to a wrong detection. %Analogously to the optimized detection, 
Figure \ref{fig:real_sequence}-e shows the components of the bounding box over the frames when only the measure of the library is used. Note how the main target is not localized correctly from frame 20 to frame 40.
 \begin{figure}[!h]
\centering
\begin{tabular}{cc}   
    \includegraphics[width=0.48\columnwidth]{images/experiment/performance/pixels/opt.jpg} 
    &
     \includegraphics[width=0.48\columnwidth]{images/experiment/performance/pixels/plot_bb_gt.jpg}
    \\
    
     \footnotesize (a)  & \footnotesize (d) 
     \\
     
    \includegraphics[width=0.48\columnwidth]{images/experiment/performance/pixels/no_opt.jpg} 
    &
     \includegraphics[width=0.48\columnwidth]{images/experiment/performance/pixels/plot_only_measure.jpg}
    \\
     \footnotesize (b)  & \footnotesize (e) 
    \\
      \includegraphics[width=0.48\columnwidth]{images/experiment/performance/depth/gt.jpg} 
    &
     \includegraphics[width=0.48\columnwidth]{images/experiment/performance/depth/plot_measure_opt.jpg}
   \\
     \footnotesize (c)  & \footnotesize (f) \\
\end{tabular}
\caption{\textbf {Analysis of the features of a frame from a real sequence.} %Measures and optimized output of the target detection module and focus detection module.
(a) Optimized output of the target localization module, with only one main target selected. Green box is ground truth and the red box is optimized output. (b) Wrong selection of the main target if the continuity between frames is not taken into account in the optimization problem. (c) Optimized output of the focus detection module. Target and Foreground are out of focus, background is in focus. (d) Optimized Bounding box of the target localization module. Light colors are ground truth and dark colors are the output. Blue lines are horizontal components and orange are vertical components (e) Not Optimized Bounding box of the target localization module. Note the misdetection in some frames compared to the ground truth values (f) Optimized output of blurry module (dark colors) together with the blurry measures in percentage (light colors). Orange is background, yellow is the target and blue is foreground and %Light colors represent the measures and dark colors represent the optimized output. 
1 is focused and 0 is not focused.}
\label{fig:real_sequence}
\end{figure}
 \begin{figure}[!h]
\centering
\begin{tabular}{cc}
    \includegraphics[width=0.48\columnwidth,height=2.1cm]{images/experiment2/pose_1.jpg} 
    &
    
     \includegraphics[width=0.48\columnwidth]{images/experiment2/keypoint.jpg}
    \\ 
    
    \footnotesize (a)  & \footnotesize (d) \\
    
    \includegraphics[width=0.48\columnwidth,height=2.1cm]{images/experiment2/pose_2.jpg} 
    &
    \includegraphics[width=0.48\columnwidth]{images/experiment2/noisy.jpg}
    \\
     \footnotesize (b)  & \footnotesize (e) \\
     
    \includegraphics[width=0.48\columnwidth,height=2.1cm]{images/experiment2/frame0.jpg} 
    &
     \includegraphics[width=0.48\columnwidth]{images/experiment2/focus.jpg}
    \\
     \footnotesize (c)  & \footnotesize (f) \\
\end{tabular}
\caption{\textbf {Analysis of the features of a frame from a simulated sequence.}(a-b) Two subsequent frames of the sequence showing the skeleton for the body joints detection algorithm (c) Focus map detected by the focus detection measure. White areas are focused, and black areas are out of focus. (d) Plot showing the ground truth (light color) and CineTransfer values for the point of the chest of the target (red middle point in skeleton). Blue are vertical components and Orange are horizontal components (e) Vertical component of the chest of the target when the continuity between frames is not optimized (light) and when it is (dark) (f) Evolution of the detected focus of the main target. Light color is the percentage of pixels detected, dark color is the optimized output, and dashed black lines are ground truth}
\label{fig:simulated_sequence}
\end{figure}

  \subsubsection{Style Transfer from a real sequence}
  The extracted features in the previous sections are converted to recording instructions that are sent to CineMPC to transfer the input style and record an output sequence that is similar to the input sequence. The sequence is first reproduced in a scenario similar to the input sequence, showing the artistic and purely aesthetic output of this solution for qualitative comparison between the two sequences. Then, the sequence is reproduced in a scenario that is very different from the input sequence for qualitative and quantitative results by comparing the output of CineTransfer in both the input and output sequences.
   \paragraph{\textbf{Qualitative results}}
The target position on the image and the focus of the scene vary along the sequence. The first three columns of Fig. \ref{fig:exp_comparing} depict three frames of the beginning, middle, and end of the sequence ordered top to bottom in time for qualitative comparison.
 First column depicts the frames of the input sequence%(from the movie Road to Perdition), 
, second column represents the same frames from the cloned sequence in a similar scenario and the third column shows the same frames recorded in a scenario that is different (football player standing up in the mountains). The frames on the bottom include a graphical representation of the points of interest of the main target for comparison. At the beginning of the sequence (first row), the main target is placed in the center and showing in focus, in the middle (second row) the target appears closer in the image and out of focus, and at the end of the sequence (third row) the target appears much closer and in focus, showing the background out of focus. Note how the cloned scenes (second and third columns) reproduce these effects qualitatively. 



\begin{figure*}[!th]
\centering
\begin{tabular}{cccc}
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/original/1.jpg} 
    &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/copy/1.jpg} 
    &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/footbal/1.jpg} 
    &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Quantitative/1.jpg} 
    \\
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/original/3.jpg} 
    &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/copy/3.jpg} 
    &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/footbal/3.jpg}  &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Quantitative/2.jpg} 
    \\
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/original/4_open.jpg} 
    &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/copy/4_open.jpg} 
    &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Qualitative/footbal/4_open.jpg}  &
    \includegraphics[width=0.24\linewidth, height=2.2cm]{images/experiment/Quantitative/3.jpg} 
    \\

    \footnotesize (a)  & \footnotesize (b) & \footnotesize (c)  & \footnotesize (d)  \\
\end{tabular}
\caption{\textbf {Comparison - Qualitative experiments}}
\label{fig:exp_comparing}
\end{figure*}

  \paragraph{\textbf{Quantitative results}}
Different plots are shown in the fourth column of Fig.~\ref{fig:exp_comparing} for quantitative comparison between the input sequence (first column) and the sequence cloned in a different scenario (third column). Both sequences are analyzed by CineTransfer to compare the results of the outputs. The results are shown in the plots, where light colors represent the values on the input sequence and dark colors represent the values on the cloned sequence. The comparison of the focus of the two sequences over frames is depicted in the first row. Yellow, orange, and blue lines represent the background, foreground, and target, respectively.
The second row represents the pixels of the bounding box of the target localized in the input sequence and the same output in the output sequence. Blue lines are vertical components and orange lines are horizontal components. Lastly, the bottom row represents the evolution of the vertical (orange) and horizontal (blue) positions of the left and right shoulders which are the parts of the body that are controlled to frame the target in this experiment. Note that the values shown in the last two rows are normalized by dividing the image position by the image height/width to support different image sensor sizes.

  \subsection{Quality of style features extracted}
\label{sec:sequence-analyze}
   %Another sequence here?
The goal of this experiment is to measure the quality of the features extracted to encode the input sequences style.
%demonstrate that this algorithm extracts the correct features from the input sequence, we validate the quality of 
We analyze
the localization of the image position and body joints of the main targets, as well as the focus of the different image regions. 

%With that aim, we use 
To have the ground truth values for these magnitudes, this experiment uses an input sequence generated in the photorealistic environment XXXX????. 

and we manually tag each frame of the real sequence with the bounding box that localizes the main target in the image and the focus of the scene. 

%Then, the values of the output of the pipeline are compared with the ground truth values in both sequences.

% Then, we perform a similar comparison of the focus, comparing tagged values with the optimized values from this solution.

%, and the focus of the scene -if the foreground, background, and target appear in focus in the image-. We then compare the values of the output with the ground truth value. Moreover, we show the potential of the optimization of the outputs by comparing the outputs of the measures not optimized with the ground truth value.
\subsubsection{Results of target and body joints localization}
%Figure \ref{fig:performance-qualitative} shows qualitative results for a determinate frame of the sequence. 
%With respect to target localization, 
 Figure~\ref{fig:raw_measures}-a depicts all the objects detected by Mask-RCNN in this frame of the real sequence. Among all the objects, three are identified as 'person' and only the main target should be selected. %CineTransfer filters and optimizes the results, localizing the target on the image  from the noisy measurement. % but only the main target should be selected.  
 Figure \ref{fig:real_sequence}-a shows the bounding box of the selected main target  in red and its ground truth in green. For quantitative results, we refer the reader to Fig. \ref{fig:real_sequence}-d, which shows 
the four components of the optimized bounding box over the frames and its ground truth. Dark and light  blue represent the horizontal ($x$) components and their ground truth, respectively.
 Analogously, dark and light orange lines represent the vertical ($y$) components. Note that the optimized values are close to the ground-truth values despite the noisy measurements, proving the correct localization of the main target.
The body joints localization performance is demonstrated by comparing the output of CineTransfer with the ground truth values of the simulated sequence. For qualitative results, Fig.\ref{fig:simulated_sequence}-a,b show two frames of the sequence with the detected skeleton. For quantitative results, Fig.\ref{fig:simulated_sequence}-d shows the 2D point of the image ($x$ is blue and $y$ is orange), normalized from 0 to 1, where the chest of the person  (red middle point in the graphical skeleton) is localized and optimized by CineTransfer over frames. Dashed lines represent ground-truth values and solid lines represent the output of the algorithm.

\subsubsection{Results of focus}
% This example shows how the optimization problem reduces the noise of the measure and predicts the correct output based on the continuity of the frames. 
The raw output of EFENet for the frames analyzed is depicted in  Fig.\ref{fig:simulated_sequence}-c for the simulated sequence and in Fig.\ref{fig:raw_measures}-b  for the real sequence.
Light areas represent the part of the scene that is in focus and dark parts are out of focus.
In the frame of the simulated sequence, the main target is the only part that is shown in focus, so the foreground and background remain out of focus. 
For quantitative results, Fig.\ref{fig:simulated_sequence}-f depicts the comparison of the percentage of focused pixels of the target optimized (dark colors) together with the raw noisy measures from the library (light color), and the ground truth values (black dashed line, 1 is focused, 0 is not focused) over frames. %Yellow, orange, and blue lines represent the focus of the background, foreground, and target, respectively. 
In the frame of the real sequence, the background is the only part that is shown in focus, so the foreground and main target remain out of focus.
Figure \ref{fig:real_sequence}-c depicts a graphical representation of the  focus of this frame optimized, which matches the ground truth value. For quantitative results, Fig.\ref{fig:real_sequence}-f depicts the comparison of the percentage of focused pixels optimized (dark colors) together with the raw noisy measures from the library (light colors) over frames. Yellow, orange, and blue lines represent the focus of the background, foreground, and target, respectively. 



%The output of EFENet extracts a boolean map that represents the pixels that are in/out of focus in a picture, which is depicted in Fig.\ref{fig:raw_measures}-b for this frame. Light areas represent the part of the scene that is in focus and dark parts are out of focus.
%In this frame, the background is the only part that is shown in focus, so the foreground and main target remain out of focus. Fig.\ref{fig:performance-qualitative}-e depicts a graphical representation of the output of CineTransfer, once optimized, which matches with the ground truth value. For quantitative results, Fig.\ref{fig:performance-qualitative}-f depicts the comparison of the percentage of focused pixels optimized (dark colors) together with the raw noisy measures from the library (light colors). Yellow, orange, and blue lines represent the focus of the background, foreground, and target, respectively. 
%Analogously, Fig.\ref{fig:performance-qualitative}d represents the evolution of the output only by taking into account the measures.


%Fig.\ref{fig:performance-qualitative}e. Figure \ref{fig:performance-quantitative}a depicts a graphical representation of the evolution of the optimized bounding box of the target along the frames of the sequence. Light blue and dark blue represent the ground truth values of the vertical components of the bounding box and the output of the optimization, respectively. Analogously, light and dark orange lines represent the horizontal components of the bounding box.

\subsubsection{The importance of the continuity term}
In this experiment, we prove how the optimization problem helps to improve the final output. %extract the output of the library if the 
In the first test, we analyze again the real sequence, but the cost term, which guarantees the continuity of the output of the bounding box of the main target ($\Theta_{f,t}$ of Eq. \ref{eq:cost-pixels}), is deactivated. Consequently, the bounding box of the main target is localized by only using the measure of the library,
\begin{equation}
\begin{aligned}
\min_{\substack{\mathbf{R}_{f,t}\\{\alpha_{f,t}}}} \quad & \sum_{f=0}^{nf}\sum_{t=0}^{nt}{\sum_{m=0}^{nm}\Pi_{f,t,m} }\\
\textrm{s.t.}
%\quad & 0 < BB_{f,t}.height < f.height \\  
%& 0 < BB_{f,t}.width < f.width  \\
 \quad & \mathbf{R}_{f,t} \in f \\
& \sum_{m=0}^{nm}{\alpha_{f,m}} = 1,  \ 0 < \alpha_{f,m}< 1 
\end{aligned}.
\end{equation}
% by setting. $w_cont$ to zero. 

Figure \ref{fig:real_sequence}-b shows the detected bounding box (red), and the expected ground truth value (green) for the analyzed frame. The optimization problem incorrectly selects the bounding box of a person that is not the main target. This might be caused because the main target appears blurry, which impacts negatively the confidence on the measure of that mask, $q_{f,m}$. The selected person appears in focus, having higher confidence, % as it appears in focus, 
and misleading to a wrong detection. %Analogously to the optimized detection, 
Figure \ref{fig:real_sequence}-e shows the components of the bounding box over the frames when only the measure of the library is used. Note how the main target is not localized correctly from frame 20 to frame 40.

Analogously, we analyze again the simulated sequence but this time, we deactivate the cost term that ensures the continuity of output of the body joints of the target over frames. In this sequence, the target is moving, so the position of the body joints varies significantly from one frame to another. Figures \ref{fig:simulated_sequence}-a and \ref{fig:simulated_sequence}-b represent this variation in two subsequent frames. The optimization problem helps to reduce this noise, providing a continuous output for a more stable framing of the target. Figure \ref{fig:simulated_sequence}-e shows the vertical component of the chest optimized (dark blue) and not optimized (light blue) normalized from 0 to 1.
Note how the optimized output is softer, reducing the noise induced by the movement of the target.



%  \begin{figure}[!h]
% \centering
% \begin{tabular}{cc}
 
%     \includegraphics[width=0.48\columnwidth]{images/experiment/performance/pixels/plot_bb_gt.jpg} 
%     &
%      \includegraphics[width=0.48\columnwidth]{images/experiment/performance/depth/plot_measure_opt.jpg}
%    \\
    
%      \footnotesize (a)  & \footnotesize (c) \\
%     \\
%        \includegraphics[width=0.48\columnwidth]{images/experiment/performance/pixels/plot_only_measure.jpg} 
%     &
%      \includegraphics[width=0.48\columnwidth]{images/4.png} \\
%      \footnotesize (b)  & \footnotesize (d) \\
% \end{tabular}
% \caption{\textbf {Quantitative experiments}- (d) ? }
% \label{fig:performance-quantitative}
% \end{figure}

  

  \subsection{Style Transfer examples from real sequences}
This experiment demonstrates how CineTransfer extracts the main features of an input sequence and gives instructions to a cinematographic platform to recreate the sequence in a similar and a different scenario. Concretely, we use CineMPC  \cite{pueyo2022cinempc}, a cinematographic platform that receives recording instructions, i.e. desired depth of field, desired position of targets in the scene, and solves an MPC optimization problem to move a drone and a camera satisfying the given instructions. We adapted CineMPC to read the CineTransfer JSON files and use them as recording instructions.
In this experiment, we reproduce the input sequence that has been analyzed in Sec. \ref{sec:sequence-analyze} in the photorealistic simulator CinemAirSim\cite{pueyo2020cinemairsim}, an extension of AirSim \cite{shah2018airsim} for cinematographic purposes. The sequence is first reproduced in a scenario similar to the input sequence, showing the artistic and purely aesthetic output of this solution for qualitative comparison between the two sequences. In the second experiment, the sequence is reproduced in a scenario that is very different from the input sequence %, but there is a main target in the scene 
for qualitative and quantitative results by comparing the output of CineTransfer in both the input and output sequences.

%is able to extract the features of a scene, independently of the scene or the scenario where the sequence is recorded.

%The idea of CineTransfer is to move a drone to recreate the features of a scene, independently of the scene or the scenario where the sequence is recorded. In this subsection, we use CineMPC\cite{pueyo2022cinempc} to obtain two output sequences in different scenarios by using the same input sequence. 

%It is important to remark, that in that solution, the localization of the targets in the scene is given for granted. First, we perform experiments in a scenario that is very similar to the one where the input sequence was recorded and compare the two sequences qualitatively, showing the artistic and purely aesthetic output of our solution. Then, we use a scenario, where there is a target, that is very different from the input sequence. In this case, we obtain qualitative and quantitative results by comparing the output of CineTransfer for both the input and output sequences.
% Salidas de blurry y de bounding box optimizando con GT
% Selección del target de interes. Mostrar qué pasa si no se optimiza, o si se desactiva el termino de continuidad. Destacar que en esta sequencia aparece mucha gente por detrás que genera ruido
% Comparar blurry con GT optimizando y sin optimizar 


  \subsubsection{Qualitative experiments}
 %The first three columns of Fig. \ref{fig:exp_comparing} depict different frames of the experiment  
 The target position on the image and the focus of the scene vary along the sequence. The first three columns of Fig. \ref{fig:exp_comparing} depict three frames of the beginning, middle, and end of the sequence ordered top to bottom in time for qualitative comparison.
 First column depicts the frames of the input sequence%(from the movie Road to Perdition), 
, second column represents the same frames from the cloned sequence in a similar scenario and the third column shows the same frames recorded in a scenario that is different (football player standing up in the mountains). The frames on the bottom include a graphical representation of the points of interest of the main target for comparison. At the beginning of the sequence (first row), the main target is placed in the center and showing in focus, in the middle (second row) the target appears closer in the image and out of focus, and at the end of the sequence (third row) the target appears much closer and in focus, showing the background out of focus. Note how the cloned scenes (second and third columns) reproduce these effects qualitatively. 
  
  
  %The qualitative experiments are depicted in the three first columns of Fig. \ref{fig:exp_comparing}. The first column represents some frames from the input sequence. The second column represents the same frames from the output sequence in the scenario that is similar to the one where the input sequence is recorded. The same frames recorded in the scenario that is different (football player standing up in the mountains) are depicted in the third column. As a guideline, the bottom frames include the output of OpenPose.

  \subsubsection{Quantitative experiments}
Different plots are shown in the fourth column of Fig.~\ref{fig:exp_comparing} for quantitative comparison between the input sequence (first column) and the sequence cloned in a different scenario (third column). Both sequences are analyzed by CineTransfer to compare the results of the outputs. The results are shown in the plots, where light colors represent the values on the input sequence and dark colors represent the values on the cloned sequence. The comparison of the focus of the two sequences over frames is depicted in the first row. Yellow, orange, and blue lines represent the background, foreground, and target, respectively.
The second row represents the pixels of the bounding box of the target localized in the input sequence and the same output in the output sequence. Blue lines are vertical components and orange lines are horizontal components. Lastly, the bottom row represents the evolution of the vertical (orange) and horizontal (blue) positions of the left and right shoulders which are the parts of the body that are controlled to frame the target in this experiment. Note that the values shown in the last two rows are normalized by dividing the image position by the image height/width to support different image sensor sizes.



